Reinforcement Learning on Variable Impedance Controller for High-Precision Robotic Assembly

Precise robotic manipulation skills are desirable in many industrial settings, reinforcement learning (RL) methods hold the promise of acquiring these skills autonomously. In this paper, we explicitly consider incorporating operational space force/torque information into reinforcement learning; this is motivated by humans heuristically mapping perceived forces to control actions, which results in completing high-precision tasks in a fairly easy manner. Our approach combines RL with force/torque information by incorporating a proper operational space force controller; where we also exploit different ablations on processing this information. Moreover, we propose a neural network architecture that generalizes to reasonable variations of the environment. We evaluate our method on the open-source Siemens Robot Learning Challenge, which requires precise and delicate force-controlled behavior to assemble a tight-fit gear wheel set.

==> sections/trim_saved.tex <==
ne can also design such force controller by directly doing simple feedback control on the difference between wrist sensor readings and desired wrenches:
\begin{equation}\label{force_pd}
\tau = g(q) + J^{T}(q)(\bF_{d} + K_{fp}\bF_{e} + K_{fi}\int\bF_{e}(t)dt),
\end{equation}
where $\bF_{e} = \bF_{d} - \bF_{tip}$, and $ K_{fp}$ and $K_{fi}$ are positive-definite gain matrices.





Compared to hard-optimality in its original cost function where only deterministic solution is possible; this soft-optimality allows solution with intermediate sub-optimal actions but ``as good as" the deterministic one with lowest cost. This so-called Maximum Entropy LQR formulation \cite{ZiebartMaxEnt} serves as an crucial step in this specific iLQG variant; it yields benefits for preparing diverse training data in aforementioned linear dynamics fitting step and training global neural network policy to be mentioned in Section \ref{nn_train}. 
